SNR-Adaptive Ranging Waveform Design Based on Ziv-Zakai Bound Optimization

Location-awareness is essential in various wireless applications. The capability of performing precise ranging is substantial in achieving high-accuracy localization. Due to the notorious ambiguity phenomenon, optimal ranging waveforms should be adaptive to the signal-to-noise ratio (SNR). In this letter, we propose to use the Ziv-Zakai bound (ZZB) as the ranging performance metric, as well as an associated waveform design algorithm having theoretical guarantee of achieving the optimal ZZB at a given SNR. Numerical results suggest that, in stark contrast to the well-known high-SNR design philosophy, the detection probability of the ranging signal becomes more important than the resolution in the low-SNR regime.

==> SupportDocuments/YF_Style_Preamble.tex <==
\newcommand{\vl}[1]{\mathbf{#1}}
\newcommand{\vg}[1]{\boldsymbol{\mathnormal{#1}}}
\newcommand{\ml}[1]{\mathbf{#1}}
\newcommand{\mg}[1]{\boldsymbol{\mathnormal{#1}}}

